DASH: A C++ PGAS Library for Distributed Data Structures and Parallel Algorithms

We present DASH, a C++ template library that offers distributed data structures and parallel algorithms and implements a compiler-free PGAS (partitioned global address space) approach. DASH offers many productivity and performance features such as global-view data structures, efficient support for the owner-computes model, flexible multidimensional data distribution schemes and inter-operability with STL (standard template library) algorithms. DASH also features a flexible representation of the parallel target machine and allows the exploitation of several hierarchically organized levels of locality through a concept of Teams. We evaluate DASH on a number of benchmark applications and we port a scientific proxy application using the MPI two-sided model to DASH. We find that DASH offers excellent productivity and performance and demonstrate scalability up to 9800 cores.

==> 00_testdrive.tex <==
% Section: Test Drive

Relevant publications from within the project:
\begin{itemize}
\item A high level description of the project's
  goals~\cite{Fuerlinger:2014:DASH}
\item DART-MPI: The MPI-3 RMA-based implementation of
  DART~\cite{Zhou:2014:DART}
\item The shared memory window optimization for
  DART-MPI~\cite{Zhou:2015:SharedMemory}
\item A CUDA-enabled implementation of DART based on the System-V
  shared memory version of DART~\cite{Zhou:2015:DARTCUDA}
\item Automatically deriving optimized data distribution patterns by
  specifying desired properties
  (make\_pattern)~\cite{Fuchs:2016:MakePattern}
\item A detailed discussion of the DASH Matrix, a \mdim array
  implementation and of the SUMMA matrix-matrix multiplication
  benchmark~\cite{Fuchs:2016:Matrix}
\end{itemize}

\subsection{A listing example}

\begin{lstlisting}[basicstyle=\footnotesize\ttfamily,frame=lines,framerule=0.5pt]
// create a distributed M x N matrix
dash::Matrix<2, double> matrix(M, N);

// select a 2D region view between
// rows r0 and r1 and columns c0 and c1
auto region = matrix.sub(0, {r0, r1})
                    .sub(1, {c0, c1});

// create local copy of region
dash::LocalCopy<double>
    lc(region.begin(), region.size());

// initiate transfer
auto res = lc.get_async();

// ... do unrelated computation

// wait for completion of transfer
res.wait();

// access local copy
lc[i] = ...;
\end{lstlisting}


